Quantum Phases and Transitions in Spin Chains with Non-Invertible Symmetries

Generalized symmetries often appear in the form of emergent symmetries in low energy effective descriptions of quantum many-body systems. Non-invertible symmetries are a particularly exotic class of generalized symmetries, in that they are implemented by transformations that do not form a group. Such symmetries appear in large families of gapless states of quantum matter and constrain their low-energy dynamics. To provide a UV-complete description of such symmetries, it is useful to construct lattice models that respect these symmetries exactly. In this paper, we discuss two families of one-dimensional lattice Hamiltonians with finite on-site Hilbert spaces: one with (invertible) $S^{\,}_3$ symmetry and the other with non-invertible $\mathsf{Rep}(S^{\,}_3)$ symmetry. Our models are largely analytically tractable and demonstrate all possible spontaneous symmetry breaking patterns of these symmetries. Moreover, we use numerical techniques to study the nature of continuous phase transitions between the different symmetry-breaking gapped phases associated with both symmetries. Both models have self-dual lines, where the models are enriched by so-called intrinsically non-invertible symmetries generated by Kramers-Wannier-like duality transformations. We provide explicit lattice operators that generate these non-invertible self-duality symmetries. We show that the enhanced symmetry at the self-dual lines is described by a 2+1D symmetry-topological-order (SymTO) of type $\mathrm{JK}^{\,}_4\boxtimes \overline{\mathrm{JK}}^{\,}_4$. The condensable algebras of the SymTO determine the allowed gapped and gapless states of the self-dual $S^{\,}_3$-symmetric and $\mathsf{Rep}(S^{\,}_3)$-symmetric models.

==> SECTIONS/app-Ising-selfdual.tex <==
\section{Ising chain with KW-symmetric deformation}
\label{app:ising self dual}

\begin{figure}[t!]
\centering
\includegraphics[height=2.1in]{FIGURES/Ising-self-dual-phase-diagram}
\ \ \ \ \ \ \ \  \ \ \  \ \ 
\ \ \ \ \ \ \ \  \ \ \  \ \ 
\ \ \ \ \ \ \ \  \ \ \  \ \ 
\ \ \ \ \ \ \ \  \ \ \  \ \ 
\\[-1.7in]
\ \ \ \ \ \ \ \  \ \ \  \ \ 
\ \ \ \ \ \ \ \  \ \ \  \ \ 
\ \ \ \ \ \ \ \  \ \ \  \ \ 
\ \ \ \ \ \ \ \  \ \ \  \ \ 
\includegraphics[height=1.5in]{FIGURES/QIsingD0_200_0_200c}\\[7mm]
\caption{Phase diagram of Hamiltonian \eqref{eq:Ham gen Ising selfdual} in the
$ (h,J) $ plane with $ \la=2-J-h $ at each point. The unshaded regions are
gapped. (Right) Tensor network computed central charge for the same range of
$(h,J,\la)$ for Ising chain of sizes
$L=256$ (blue),
$L=128$ (green),
$L=64$ (red).
The stripe pattern in the gapless
$c\neq 0$ area comes from incommensurate nature of the gapless phase.
The $h=J$ line has self-dual symmetry.
} \label{fig:ising-self-dual-phase-diagram}
\end{figure}

It is instructive to study the phase diagram of the following Hamiltonian
\begin{align}
\widehat{H}
\=
-
\sum_{j=1}^{N}
\left\{
J\,
\hat{\sigma}^{z}_{j}\,
\hat{\sigma}^{z}_{j+1}
+
h\,\hat{\sigma}^{x}_{j}
+
\lambda
(
\hat{\sigma}^{y}_{j}\,
\hat{\sigma}^{z}_{j+1}
-
\hat{\sigma}^{z}_{j}\,
\hat{\sigma}^{y}_{j+1}
)
\right\},
\label{eq:Ham gen Ising selfdual}
\end{align}
which is the transverse field Ising model perturbed by a Dzyaloshinskii-Moriya-type
interaction. The latter is one of the simplest two-body interactions 
that is symmetric under the (non-invertible) Kramers-Wannier symmetry of
the critical point of the Ising model.
The model can be solved exactly by mapping to a fermionic Hamiltonian with
only quadratic interactions by JW transformation~\Rf{SCL09051849}.
After the JW transformation, one can diagonalize the fermionic Hamiltonian
via a Bogoliubov transformation which yields
\begin{equation}\label{eq:Ham fermion}
\widehat{H} 
= 
\sum_{-\pi< k\leq \pi} 
E^{\,}_k \, 
\hat{\psi}_k^{\dagger} \hat{\psi}^{\,}_k + E^{\,}_0
\end{equation}
where
\begin{equation}\label{eq:Ek fermion}
E^{\,}_k = 
4\lambda \sin k 
\pm 
2\sqrt{J^2\sin^2 k+(h-J\cos k)^2}
\end{equation}
Here, we note that electrons at quasi-momentum $ k $ 
are identified with holes at quasi-momentum $ -k $. 
We can either choose to only look at both electrons and holes 
for quasi-momenta in $ [0,\pi] $ or only the electrons 
(or, equivalently only the holes) for all $ k\in (-\pi,\pi] $. 
We take the latter point of view.


From the above spectrum, we can identify the low-energy degrees 
of freedom and whether the ground state is gapped or not. 
Whenever there are linear dispersing modes 
at zero energy with left and right moving partners, 
we interpret the low energy effective field theory as a $ c=1/2 $ 
Majorana CFT. Whenever there are two 
pairs of such linear dispersing modes, we identify 
the low energy effective field theory to be a $ c=1 $ compact boson theory. 
The phase diagram we obtain from this analysis is 
shown in \fig{fig:ising-self-dual-phase-diagram}.

The extended gapless regions labeled $ c=1 $ have 
gapless linear-dispersing modes at wavenumbers 
that smoothly vary throughout those regions. 
This behavior is seen only when $ \la $ 
is larger than $ \approx 0.4 $ or smaller than $ \approx -0.66 $. 
Moreover, we see that the Ising CFT is actually stable 
to a finite non-zero value of $ \la $. This motivates 
us to draw analogies with the behavior seen in our 
$ S^{\,}_{3} $ and $ \cRep(S^{\,}_{3}) $ symmetric Hamiltonians, 
\eqref{eq:Ham gen S3 reparameterized} and 
\eqref{eq:Ham gen Rep S3 reparameterized}, where the critical
lines and the multi-critical point are found to be stable to turning on 
finite non-zero values of $ \th $. 
The parameter $ \th $ in these models 
plays a very similar role to that of $ \la $ in the deformed Ising model above.
At large enough values of $ \th $ and $ \la $ in respective models,
a \emph{sliding density-wave} phase appears. 




==> SECTIONS/discussion240505.tex <==
\section{Discussion}
\label{sec:disc}

Let us recap and give a detailed discussion of the main lessons from Secs.\
\ref{sec:S3model} and \ref{sec:RepS3model}.  We collect our key results under
three directions.  Sec.\ \ref{sec:discussion gauging dualities} reviews the web
of dualities we have obtained by gauging various subgroups of $S^{\,}_{3}$.  In
Sec.\ \ref{subsec:correlation funcs}, we describe symmetry-breaking patterns in
terms of patch operators, and compute their expectation values in the gapped
fixed-point ground states. We argue that these can be used to detect  ordered
and disordered phases of models with general fusion category symmetries.
Finally, Sec.\ \ref{sec:SymTO analysis} complements our discussion of gapped
phases of $S^{\,}_{3}$ and $\cRep(S^{\,}_{3})$ symmetries from the perspective
of symmetry topological order (SymTO) correspondence.

\subsection{Gauging-induced dualities}
\label{sec:discussion gauging dualities}

In Secs.\ \ref{sec:S3model} and \ref{sec:RepS3model}, we presented several
dualities that are induced by gauging subgroups of $S^{\,}_{3}$ symmetry.  In
Fig.\ \ref{fig:duality web}, we summarize the corresponding web of dualities.
The corners of the diagram label the symmetry categories of the dual bond
algebras while the each arrow implies a duality map induced by gauging. It has
been shown in Ref.\ \cite{BT170402330}, distinct gaugings of a symmetry
category $\mathcal{C}$ are in one-to-one correspondence with the left (or
right) module categories over $\mathcal{C}$. Accordingly, we label each arrow
in Fig.~\ref{fig:duality web} by the choice of the corresponding module
category.\footnote{Module categories over $\cVec_G$ ($\cRep(G)$) are given by
the categories $\cVec_H$ ($\cRep(H)$) where $H \leqslant G$, \ie $H$ is a
subgroup of G~\cite{EGNV16}.} Alternatively, each left (or right) module
category over $\mathcal{C}$ is equivalent to the category of right (or left)
$A$-modules over $\mathcal{C}$ where $A\in \mathcal{C}$ is some algebra object
(see Appendix A of Ref.\ \cite{CRBSS230509713}).  This correspondence forms the
connection between the module categories over $\mathcal{C}$ and the perspective
on gauging as summing over symmetry defect insertions in two-dimensional
spacetime.  In the context of fusion category symmetries, gauging can then be
understood as summing over all insertions of $A$-defects in the partition
function in two-dimensional spacetime.

\begin{figure}[t] \centering
\includegraphics[width=0.6\linewidth]{FIGURES/duality_summary} \caption{The web
of dualities obtained induced by gauging.  The four categories $\cVec_{S_{3}}$,
$\cVec_{S^{\vee}_{3}}$, $\cRep(S^{\,}_{3})$, and $\cRep(S^{\vee}_{3})$ at the
corners of the diagram denote the fusion category symmetry of the bond algebras
\eqref{eq:def S3 algebra}, \eqref{eq:def S3/Z3 algebra}, \eqref{eq:def S3/Z2
algebra}, and  \eqref{eq:def S3/S3 algebra}, respectively.  Each directed arrow
between these fusion categories denote a duality induced by gauging. The label
on each arrow denotes the corresponding module category over the category at
the source of the arrow. } \label{fig:duality web} \end{figure}

In \fig{fig:duality web}, for the fusion category
$\cVec_{S^{\,}_{3}}$,\footnote{For any group $G$, the fusion category $\cVec_G$
consists of simple objects that can be thought of as $G$-graded vector spaces,
which fuse according to group multiplication law. The morphisms of this
category are graded $G$-graded linear maps. In this subsection, we will refer
to $S_3$ symmetry as $\cVec_{S^{\,}_{3}}$ to emphasize the general language of
fusion category symmetry.} the module categories label the symmetry category of
the subgroups that are not gauged. Note that the module categories are in
one-to-one correspondence with (conjugacy classes) of subgroups of $S^{\,}_3$.
In particular, the module categories $\cVec_{S^{\,}_{3}}$ and
$\cVec_{\Z^{\,}_2}$ of $\cVec_{S^{\,}_{3}}$ correspond to gauging by the
algebra objects $e$ (the trivial algebra object, implementing trivial gauging)
and $e\oplus r\oplus r^2$, respectively. These gauging maps give back the same
symmetry category $\cVec_{S^{\,}_{3}}$.  The latter, in particular, is what we
would ordinarily describe as the $\Z^{\,}_3$ Kramers-Wannier duality. We
provided a recipe for implementing this gauging map in \scn{sec:gauging Z3 in
S3}. On the other hand, the module categories $\cVec_{\Z^{\,}_3}$ and
$\cVec_{\Z_1}$, where $\Z_1$ is the trivial group, correspond to gauging
$\cVec_{S^{\,}_{3}}$ by the algebra objects $e\oplus s$ and $e\oplus r\oplus
r^2\oplus s \oplus sr \oplus sr^2$, respectively. These gauging maps lead to
the dual $\cRep(S^{\,}_{3})$ symmetry category. The first of these is exactly
the gauging map we used to construct the $\cRep(S^{\,}_{3})$ spin chain in
\scn{sec:RepS3model}, starting from the $S^{\,}_{3}$ spin chain of
\scn{sec:S3model}. The second one of these can be implemented by first gauging
$\Z^{\,}_3$ in $S^{\,}_{3}$ and then gauging the $\Z^{\,}_2$ subgroup of the
dual $S^{\vee}_3$, as discussed in \scn{sec:gauging S3 in S3}.

For the fusion category $\cRep(S^{\,}_{3})$, we find that the algebra objects
corresponding to three distinct gaugings of $\cRep(S^{\,}_{3})$ labeled by
module categories $\cRep(\mathbb{Z}^{\,}_{3})$, $\cRep(\mathbb{Z}^{\,}_{2})$,
and $\cRep(\mathbb{Z}^{\,}_{1})$ to be $\bm{1}\oplus\bar{\bm{1}}$,
$\bm{1}\oplus\bm{2}$, and $\bm{1}\oplus\bar{\bm{1}}\oplus2\,\bm{2}$,
respectively.\footnote{These were derived using the internal Hom construction
outlined in Appendix A.3 of \Rf{CRBSS230509713}.} Gauging by certain algebra
objects can give back the same symmetry category. For other algebra objects,
one gets a new (dual) symmetry category.  This is a generalization of
Kramers-Wannier duality to arbitrary fusion category symmetries.  In our
example with $\cRep(S^{\,}_{3})$ symmetry, we find that gauging by either of
the algebra objects $\bm{1}\oplus\bar{\bm{1}}$ or
$\bm{1}\oplus\bar{\bm{1}}\oplus2\,\bm{2}$ (\ie the regular representation
object) of $\cRep(S^{\,}_3)$ gives rise to $S^{\,}_3$ symmetry.  On the other
hand, gauging by either the trivial algebra object $\bm 1$ (\ie implementing
trivial gauging) or the algebra object $\bm{1}\oplus\bm{2}$ gives back a
``dual" $\cRep(S^\vee_3)$ symmetry. Like the familiar KW duality associated
with gauging Abelian groups, the gauging by $\bm{1}\oplus\bm{2}$ implements a
duality transformation that exchanges pairs of gapped phases of the system. In
our analysis, we did not provide an explicit description of how gauging by
algebra objects, via the insertion of defects approach put forward in
\Rf{BT170402330}, works at the level of microscopic Hamiltonians. However, we
note that gauging by the $\bm{1}\oplus\bar{\bm{1}}$ algebra object should
proceed very identically to gauging of an ordinary $\Z^{\,}_2$ symmetry since
$\widehat{W}_{\bar{\bm 1}}$ indeed generates a $\Z^{\,}_2$ sub-symmetry of
$\cRep(S^{\,}_{3})$, and gauging by the regular representation algebra object
should be identical to first gauging by $\bm{1}\oplus\bar{\bm{1}}$ and then
gauging the $\Z^{\,}_3$ subgroup of the resulting $S^{\,}_{3}$ symmetry.
Finally, we identify a sequential quantum circuit \eqref{eq: def DRepS3}, that
implements a duality transformation of our $\cRep(S^{\,}_{3})$ spin chain,
which therefore must correspond to the remaining option of gauging by the
$\bm{1}\oplus\bm{2}$ algebra object. 


\subsection{SSB patterns and order/disorder operators}
\label{subsec:correlation funcs}

\setlength{\tabcolsep}{4pt} \renewcommand{\arraystretch}{1.5} \begin{table}
\caption{ \label{tab:S3 order and disorder ops GS} Expectation values of
$S^{\,}_{3}$ order and disorder operators defined in Eq.\ \eqref{eq:S3 order
disorder ops} in the fixed point ground state wavefunctions defined in Eqs.\
\eqref{eq:GS S3}, \eqref{eq:GS Z3}, \eqref{eq:GS Z2}, and \eqref{eq:GS Z1},
respectively.  The non-zero (zero) expectation values of order (disorder)
operators detect the spontaneous symmetry breaking and long-range order in the
ground states.  } \centering \begin{tabular}{l|cccc} \hline \hline $\text{GS}$
& $\widehat{C}^{\,}_{\Z^{\,}_2}(j,\ell)$ & $\widehat{U}^{\,}_{[s]}(j,\ell)$ &
$\widehat{C}^{\,}_{\Z^{\,}_3}(j,\ell)$ & $\widehat{U}^{\,}_{[r]}(j,\ell)$ \\
\hline $\ket{\mathrm{GS}^{\,}_{S^{\,}_{3}}}$ & $0$ & $+3$ & $0$ & $+2$ \\
$\ket{\mathrm{GS}^{\pm}_{\Z^{\,}_{3}}}$ & $+1$ & $0$ & $0$ & $+2$ \\
$\ket{\mathrm{GS}^{\alpha}_{\Z^{\,}_{2}}}$ & $0$ & +1 & $+2$ & $0$ \\
$\ket{\mathrm{GS}^{\pm,\alpha}_{\Z^{\,}_{1}}}$ & $+1$ & $0$ & $+2$ & $0$ \\
\hline \hline \end{tabular} \end{table} \renewcommand{\arraystretch}{1}

Ordered phases in which symmetries are spontaneously broken can be detected by
non-zero values of appropriate correlation functions of order operators.  In
contrast, disordered phases can be detected by non-zero values of appropriate
correlation functions of disorder operators.  The expectation values of
correlation functions of order and disorder operators, considered together,
have been found to be a tool that can detect gaplessness \Rf{L190309028}. The
idea of order and disorder operators can be generalized to non-invertible
symmetries in the form of patch operators
\cite{JW191213492,CW220303596,IW231005790}.  Depending on which gapped phase
the system is in, different patch operators will get a non-zero expectation
value in the ground state(s).  This gives a way to detect symmetry-breaking
even if we restrict to the symmetric sub-Hilbert space so that ground state
degeneracy is no longer a reliable tool.

For the $S^{\,}_{3}$ symmetry, we have the patch operators~\footnote{ We
choose, without loss of generality, $\hat{\si}^z_j \,\hat{\si}^z_{j+\ell}$ to
be the $\Z^{\,}_{2}$ order operator. Alternatively, we could have chosen
$\hat{\si}^z_j \,\hat{\tau}^z_{j+\ell}$, $\hat{\tau}^z_j
\,\hat{\si}^z_{j+\ell}$, or $\hat{\tau}^z_j \,\hat{\tau}^z_{j+\ell}$ as well.
Any of these choices for the order operators produce the same expectation
values in the ground states of gapped fixed-points of the Hamiltonian
\eqref{eq:Ham gen S3 reparameterized}.  } \begin{subequations} \label{eq:S3
order disorder ops} \begin{align} \widehat{C}^{\,}_{\Z^{\,}_2}(j,\ell) \=
\hat{\si}^z_j \,\hat{\si}^z_{j+\ell}, \qquad
\widehat{C}^{\,}_{\Z^{\,}_3}(j,\ell) \= \widehat{Z}^{\,}_j \
\widehat{Z}^{\dagger}_{j+\ell} + \widehat{Z}^{\dagger}_j \
\widehat{Z}^{\,}_{j+\ell}, \end{align} that are associated with $\Z^{\,}_{2}$
and $\Z^{\,}_{3}$ order operators, respectively, and the patch operators
\begin{align} \widehat{U}^{\,}_{[s]}(j,\ell) \= \sum_{\alpha=0}^{2}
\prod_{k=j}^{j+\ell}
\hat{\si}^x_k\,\hat{\tau}^x_k\,\widehat{C}^{\,}_k\,\widehat{X}^{\alpha}_{k},
\qquad \widehat{U}^{\,}_{[r]}(j,\ell) \= \prod_{k=j}^{j+\ell}
\widehat{X}^{\,}_k + \prod_{k=j}^{j+\ell}  \widehat{X}^{\dagger}_k, \end{align}
\end{subequations} that are associated with $\Z^{\,}_{2}$ and $\Z^{\,}_{3}$
disorder operators, respectively.  We note that both of these classes of patch
operators are symmetric under the entire $S^{\,}_{3}$ group, i.e., they are
constructed out of the generators of $S^{\,}_{3}$-symmetric bond algebra
\eqref{eq:def S3 algebra}, while the disorder operators are closed under the
action of $S^{\,}_{3}$.  Both order and disorder operators can be thought of as
\textit{transparent} patch operators \cite{CW220303596} in the sense that they
commute all the terms in the $S^{\,}_{3}$ Hamiltonian \eqref{eq:Ham gen S3
reparameterized} that are supported between sites $j+1$ and $j+\ell-1$.  On the
Hamiltonian their nontrivial actions only appear at their boundaries.

The expectation values attained by the patch operators in the gapped
fixed-point  ground states \eqref{eq:GS S3}, \eqref{eq:GS Z3}, \eqref{eq:GS
Z2}, and \eqref{eq:GS Z1} are given in Table \ref{tab:S3 order and disorder ops
GS}.  In the fixed-point ground states, non-zero expectation values of order
operators accompany the vanishing expectation values of disorder operators and
detect spontaneous symmetry breaking in the ground states.  We note that when
the group $S^{\,}_{3}$ is broken down to $\mathbb{Z}^{\,}_{2}$, each of the
threefold degenerate ground states preserve a different $\mathbb{Z}^{\,}_{2}$
subgroup which reflected in the non-vanishing expectation value of
$\mathbb{Z}^{\,}_{2}$ disorder operators on only one of the degenerate ground
states. Away from the fixed-points the zero expectation values are expected to
be replaced by an exponential decay $\propto e^{-|j-\ell|/\xi}$ with a finite
non-zero correlation length $\xi$ (with gapped fixed-points corresponding to
$\xi\to 0$ limit).

\setlength{\tabcolsep}{4pt} \renewcommand{\arraystretch}{1.5} \begin{table}
\caption{ \label{tab:repS3 order and disorder ops GS} Expectation values of
$\cRep(S^{\,}_{3})$ order and disorder operators defined in Eq.\
\eqref{eq:repS3 order disorder ops} in the fixed point ground state
wavefunctions defined in Eqs.\ \eqref{eq:GS repS3}, \eqref{eq:GS W1},
\eqref{eq:GS W2}, \eqref{eq:gs12}, and \eqref{eq:gs3}, respectively.  The
non-zero (zero) expectation values of order (disorder) operators detect the
spontaneous symmetry breaking and long-range order in the ground states.  }
\centering \begin{tabular}{l|cccc} \hline \hline $\text{GS}$ &
$\widehat{C}^{\,}_{\mathbf{\bar{1}}}(j,\ell)$ &
$\widehat{W}^{\,}_{\mathbf{\bar{1}}}(j,\ell)$ &
$\widehat{C}^{\,}_{\mathbf{2}}(j,\ell)$ &
$\widehat{W}^{\,}_{\mathbf{2}}(j,\ell)$ \\ \hline
$\ket{\mathrm{GS}^{\,}_{\cRep(S^{\,}_{3})}}$ & $0$ & $+1$ & $0$ & $+2$ \\
$\ket{\mathrm{GS}^{\alpha}_{\mathbf{\bar{1}}}}$ & $0$ & $+1$ & $+2$ & $0$ \\
$\ket{\mathrm{GS}^{\pm}_{\mathbf{2}}}$ & $+3$ & $0$ & $0$ & $+2$ \\
$\ket{\mathrm{GS}^{\pm}_{\mathbf{1}}}$ & $+1$ & $0$ & $+2$ & $0$ \\
$\ket{\mathrm{GS}^{3}_{\mathbf{1}}}$ & $+1$ & $0$ & $+2$ & $0$ \\ \hline \hline
\end{tabular} \end{table} \renewcommand{\arraystretch}{1}

For the $\cRep(S^{\,}_{3})$ symmetry, we can apply the $\mathbb{Z}^{\,}_{2}$
gauging map, derived in Sec.\ \ref{sec:RepS3model}, to obtain the
$\cRep(S^{\,}_{3})$ patch operators.  Since we are gauging $\Z^{\,}_{2}$
subgroup of $S^{\,}_{3}$, we expect the $\mathbb{Z}^{\,}_{2}$ order and
disorder operators to be mapped to disorder and order operators of the dual
$\Z^{\,}_{2}$ symmetry generated by $\widehat{W}^{\,}_{\mathbf{\bar{1}}}$
operator.  Accordingly, we identify the patch operators \begin{subequations}
\label{eq:repS3 order disorder ops} \begin{align} &
\widehat{C}^{\,}_{\mathbf{\bar{1}}}(j,\ell) \= \hat{\mu}^{z}_{j}\,
\sum_{\al=0}^2 \left( \prod_{k=j}^{j+\ell}
\widehat{X}^{\prod_{q=j+1}^{k}\hat{\mu}^{x}_{q}}_{k} \right)^\al
\hat{\mu}^{z}_{j+\ell},
% \hat{\mu}^{z}_{j}\, \left( 1 + \prod_{k=j}^{j+\ell}
% \widehat{X}^{\prod_{q=j+1}^{k}\hat{\mu}^{x}_{q}}_{k} + \prod_{k=j}^{j+\ell}
% \widehat{X}^{-\prod_{q=j+1}^{k}\hat{\mu}^{x}_{q}}_{k} \right)
% \hat{\mu}^{z}_{j+\ell},
\\ & \widehat{W}^{\,}_{\mathbf{\bar{1}}}(j,\ell) \= \prod_{k=j+1}^{j+\ell}
\hat{\mu}^{x}_{k}, \end{align} that correspond to
$\widehat{W}^{\,}_{\mathbf{\bar{1}}}$ order and disorder operators,
respectively.  In contrast to this, under gauging $\mathbb{Z}^{\,}_{2}$
subgroup of $S^{\,}_{3}$ symmetry, the $\Z^{\,}_{3}$ order and disorder
operators are mapped to \begin{align} & \widehat{C}^{\,}_{\mathbf{2}}(j,\ell)
\= \widehat{Z}^{\prod_{k=j+1}^{j+\ell}\hat{\mu}^{x}_{k}}_{j}\,
\widehat{Z}^{\dagger}_{j+\ell} +
\widehat{Z}^{-\prod_{k=j+1}^{j+\ell}\hat{\mu}^{x}_{k}}_{j}\,
\widehat{Z}^{\,}_{j+\ell}, \\ & \widehat{W}^{\,}_{\mathbf{2}}(j,\ell) \=
\prod_{k=j}^{j+\ell} \widehat{X}^{\prod_{q=j+1}^{k}\hat{\mu}^{x}_{q}}_{k} +
\prod_{k=j}^{j+\ell} \widehat{X}^{-\prod_{q=j+1}^{k}\hat{\mu}^{x}_{q}}_{k},
\end{align} \end{subequations} which are the order and disorder operators,
respectively, associated with the non-invertible symmetry operator
$\widehat{W}^{\,}_{\mathbf{2}}$.  We note that for $\cRep(S^{\,}_{3})$
symmetry, order operators are non-local string-like objects, as opposed to the
case of $S^{\,}_{3}$ symmetry for which order operators are bilocal, i.e.,
products of two local operators. In other words, the spontaneous breaking of
non-invertible $\cRep(S^{\,}_{3})$ is detected by non-local string order
parameters.  The expectation values attained by the patch operators in the
gapped fixed-point ground states \eqref{eq:GS repS3}, \eqref{eq:GS W1},
\eqref{eq:GS W2}, and \eqref{eq:GS 1} are given in Table~\ref{tab:repS3 order
and disorder ops GS}.  We see that the expectation values of operators
\eqref{eq:repS3 order disorder ops} in these ground states are consistent with
interpreting the corresponding phases as $\cRep(S^{\,}_{3})$-symmetric,
$\cRep(S^{\,}_{3})/\mathbb{Z}^{\,}_{2}$ SSB, $\mathbb{Z}^{\,}_{2}$ SSB, and
$\cRep(S^{\,}_{3})$ SSB phases, respectively.

\subsection{SymTO perspective} \label{sec:SymTO analysis}

The symmetry data of a 1+1d bosonic system with $ S^{\,}_{3} $ symmetry can be
encapsulated more completely in its symmetry-topological order
(SymTO)\footnote{SymTO was referred to as ``categorical symmetry'' in some
early papers. Such ``categorical symmetry'' ({\it i.e.} SymmTO) was referred to
as SymTFT later, and nowadays, categorical symmetry is used to referred to
non-invertible symmetry.},\cite{JW191213492} which is $ \cD(S^{\,}_{3}) $, the
$ S^{\,}_{3} $ quantum double, \ie $S^{\,}_3$ topological order in
2+1d.\footnote{See Appendix \ref{app:SymTO} for a review of SymTO.} From this
point of view, we \cite{KZ200514178,CW220506244} argued that the gapped phases
allowed by $ S^{\,}_{3} $ symmetry are in one-to-one correspondence to the
gapped boundaries of the SymTO $\cD(S^{\,}_{3})$.\footnote{Similar statements
have also appeared elsewhere in the
literature.\cite{MMT220710712,ZC230401262,BBS231003784}} 

It turns out that $S^{\,}_{3}$-symmetry and $ \cRep(S^{\,}_{3}) $-symmetry are
holo-equivalent, in the sense that the corresponding $S^{\,}_{3}$-symmetric
model and $ \cRep(S^{\,}_{3}) $-symmetric model are identical when restricted
to the corresponding symmetric sub-Hilbert space.  As a result,
$S^{\,}_{3}$-symmetric model and $ \cRep(S^{\,}_{3}) $-symmetric model have
identical phase diagram and phases transitions.  However, the corresponding
phases and phase transitions may be given different names.  Both of
$S^{\,}_{3}$-symmetry and $ \cRep(S^{\,}_{3}) $-symmetry have the same SymTO
(and thus holo-equivalent), as can be verified by computing the algebra of the
associated patch operators; some related examples were discussed in
\Rfs{CW220303596,IW231005790}. 

The $\cD(S^{\,}_{3})$ symTO has eight types of point-like excitations, whose
topological spins $s$, quantum dimensions $d$, $S$-matrix, and fusion rule are
given below
\begin{align}
&\ \ \ \ 
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
$\cD(S^{\,}_{3})$ & $\one$ 
& $\one'$ 
& $\two$ 
& $r$ 
& $r_1$ 
& $r_2$ 
& $s$ 
& $s_1$ 
\\ 
\hline
$s$: & $0$
& $0$
& $0$
& $0$
& $\frac{1}{3}$
& $\frac{2}{3}$
& $0$
& $\frac{1}{2}$
\\ 
\hline
$d$: & $1$
& $1$
& $2$
& $2$
& $2$
& $2$
& $3$
& $3$
\\ 
\hline
\end{tabular}
\nonumber\\
 S= & \begin{pmatrix}
1,
& 1,
& 2,
& 2,
& 2,
& 2,
& 3,
& 3 \\ 
1,
& 1,
& 2,
& 2,
& 2,
& 2,
& -3,
& -3 \\ 
2,
& 2,
& 4,
& -2,
& -2,
& -2,
& 0,
& 0 \\ 
2,
& 2,
& -2,
& 4,
& -2,
& -2,
& 0,
& 0 \\ 
2,
& 2,
& -2,
& -2,
& -2,
& 4,
& 0,
& 0 \\ 
2,
& 2,
& -2,
& -2,
& 4,
& -2,
& 0,
& 0 \\ 
3,
& -3,
& 0,
& 0,
& 0,
& 0,
& 3,
& -3 \\ 
3,
& -3,
& 0,
& 0,
& 0,
& 0,
& -3,
& 3 \\ 
\end{pmatrix}
\\
&
\hskip -13mm
{\small
\begin{tabular}{ |c||c|c|c|c|c|c|c|c|}
 \hline 
 & $\one$  & $\one'$  & $\two$  & $r$  & $r_1$  & $r_2$  & $s$  & $s_1$ \\ 
\hline 
 \hline 
$\one$  & $ \one$  & $ \one'$  & $ \two$  & $ r$  & $ r_1$  & $ r_2$  & $ s$  & $ s_1$  \\ 
 \hline 
$\one'$  & $ \one'$  & $ \one$  & $ \two$  & $ r$  & $ r_1$  & $ r_2$  & $ s_1$  & $ s$  \\ 
 \hline 
$\two$  & $ \two$  & $ \two$  & $ \one \oplus \one' \oplus \two$  & $ r_1 \oplus r_2$  & $ r \oplus r_2$  & $ r \oplus r_1$  & $ s \oplus s_1$  & $ s \oplus s_1$  \\ 
 \hline 
$r$  & $ r$  & $ r$  & $ r_1 \oplus r_2$  & $ \one \oplus \one' \oplus r$  & $ \two \oplus r_2$  & $ \two \oplus r_1$  & $ s \oplus s_1$  & $ s \oplus s_1$  \\ 
 \hline 
$r_1$  & $ r_1$  & $ r_1$  & $ r \oplus r_2$  & $ \two \oplus r_2$  & $ \one \oplus \one' \oplus r_1$  & $ \two \oplus r$  & $ s \oplus s_1$  & $ s \oplus s_1$  \\ 
 \hline 
$r_2$  & $ r_2$  & $ r_2$  & $ r \oplus r_1$  & $ \two \oplus r_1$  & $ \two \oplus r$  & $ \one \oplus \one' \oplus r_2$  & $ s \oplus s_1$  & $ s \oplus s_1$  \\ 
 \hline 
$s$  & $ s$  & $ s_1$  & $ s \oplus s_1$  & $ s \oplus s_1$  & $ s \oplus s_1$  & $ s \oplus s_1$  & $ \one \oplus \two \oplus r \oplus r_1 \oplus r_2$  & $ \one' \oplus \two \oplus r \oplus r_1 \oplus r_2$  \\ 
 \hline 
$s_1$  & $ s_1$  & $ s$  & $ s \oplus s_1$  & $ s \oplus s_1$  & $ s \oplus s_1$  & $ s \oplus s_1$  & $ \one' \oplus \two \oplus r \oplus r_1 \oplus r_2$  & $ \one \oplus \two \oplus r \oplus r_1 \oplus r_2$  \\ 
 \hline 
\end{tabular}
}
\nonumber 
\end{align}
We may view $S_3 = \Z_3\rtimes \Z_2$, where $\Z_3$ is generated by $2\pi/3$
rotations $r$ and $\Z_2$ is generated by $y\to -y$ reflection $s$.  The
particle $\one'$ is the 1-dimensional representation of $\Z_3\rtimes \Z_2$ and
can be viewed as the $\Z_2$ charge.  From the $S$ matrix, we see that moving
particle $\one'$ around particle $s$ generates $-1$, and thus $s$ is the $\Z_2$
flux.

There are four Lagrangian condensable algebras of $ \cD(S^{\,}_{3}) $. These
Lagrangian algebras describe gapped boundaries obtained by condensing various
subsets of mutually trivially braiding bosonic anyons of $\cD(S^{\,}_{3})$ on a
1+1d boundary of the topologically ordered 2+1d bulk phase. The four Lagrangian
algebras of $\cD(S^{\,}_{3})$ are denoted as follows: 
\begin{enumerate}[(i)]
\item $\cA_1 = \one \oplus \one' \oplus 2 \two $ corresponds to $S^{\,}_{3}$ SSB
completely ($S^{\,}_{3}$ ferromagnet) 
\item $\cA_2 = \one \oplus \one' \oplus 2 r$ corresponds to $S^{\,}_{3}$ SSB to $\Z^{\,}_3$ \item $\cA_3 = \one \oplus \two \oplus s $ corresponds to $S^{\,}_{3}$ SSB to $\Z^{\,}_2$ 
\item $\cA_4 = \one \oplus r \oplus s $ corresponds to $S^{\,}_{3}$ symmetric phase
($S^{\,}_{3}$ paramagnet) 
\end{enumerate} 
Here we have noted which gapped
$S^{\,}_{3}$-symmetric phase each of the Lagrangian algebra corresponds to.

In terms of the holo-equivalent $\cRep(S^{\,}_{3})$ symmetry, the first one is
the symmetric gapped phase while the last one is one that corresponds to a
completely symmetry broken phase. The other two are more subtle, and we
investigate a lattice model with $\cRep(S^{\,}_{3})$ symmetry below to better
understand the symmetry-breaking patterns of these phases better.  We find that
the second one is only symmetric under a $\cRep(\Z^{\,}_2)$ sub-fusion category
symmetry of $\cRep(S^{\,}_{3})$, while the third one breaks this
$\cRep(\Z^{\,}_2)$ while respecting the symmetry of $\cRep(S^{\,}_{3})$
associated with the element $\mathbf{2}$.

In \Rf{CW220506244}, the authors also highlighted the importance of a duality
associated with the permutation of the anyons $\two$ and $r$, which is the
automorphism of $\cD(S^{\,}_{3})$.  Here, we would like stress an important
difference of $\cD(S^{\,}_{3})$ SymTO and $\cD(S^{\,}_{3})$ SymTFT.

In $\cD(S^{\,}_{3})$ SymTFT, the automorphism $\two \leftrightarrow r$ implies
a symmetry of SymTFT.  In contrast, $\cD(S^{\,}_{3})$ SymTO is just an 2+1D
$S_3$ lattice gauge theory with matter.  Thus in general, the SymTO ({\it i.e.}
the lattice gauge theory) does not have any symmetry.  This correspond to the
fact that our $S_3$ and $\cRep(S^{\,}_{3})$ lattice models, in general, do not
have the self-dual symmetry, and their SymTO is the $\cD(S^{\,}_{3})$ SymTO
(without the $\two \leftrightarrow r$ automorphism symmetry $\Z^{\two
\leftrightarrow r}_2$).

However, the presence of $\two \leftrightarrow r$ automorphism implies that we
can fine tune the  $\cD(S^{\,}_{3})$ SymTO to make it to have the automorphism
symmetry $\Z^{\two \leftrightarrow r}_2$.  This, in turn, implies that we can
fine tune the  $S_3$ and $\cRep(S^{\,}_{3})$ lattice models, so that the
fine-tuned models have a  self-dual symmetry.  In this paper, we explicitly
constructed such lattice self-dual symmetry explicitly.

The fine-tuned lattice models have a larger symmetry which include both the
self-dual symmetry and one of the $S_3$ or $\cRep(S^{\,}_{3})$ symmetries.
Thus, the fine-tuned lattice models have a larger SymTO.  Such a larger SymTO
can be obtained by gauging the $\Z_2^{\two \leftrightarrow r}$ automorphism
symmetry in $\cD(S^{\,}_{3})$ SymTO.  This gives us the larger SymTO, which is
$SU(2)_4\times \overline{SU(2)}_4$ or $JK_4\times \overline{JK}_4$ topological
orders.  The two-fold amiguity comes from the possibility of the stacking a
$\Z_2^{\two \leftrightarrow r}$ SPT state to the SymTO, before the $\Z_2^{\two
\leftrightarrow r}$ gauging.  The anyon data for the $SU(2)_4\times
\overline{SU(2)}_4$ and $JK_4\times \overline{JK}_4$ topological orders are
given below:
\begin{align}
&\ \ \ \ 
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$SU(2)_4$& $\one$ 
& $e$ 
& $m$ 
& $m_1$ 
& $q$ 
\\ 
\hline
$s$: & $0$
& $0$
& $\frac{1}{8}$
& $\frac{5}{8}$
& $\frac{1}{3}$
\\ 
\hline
$d$: & $1$
& $1$
& $\sqrt{3}$
& $\sqrt{3}$
& $2$
\\ 
\hline
\end{tabular}
\nonumber\\
S=&\begin{pmatrix}
1,
& 1,
& \sqrt{3},
& \sqrt{3},
& 2 \\ 
1,
& 1,
& -\sqrt{3},
& -\sqrt{3},
& 2 \\ 
\sqrt{3},
& -\sqrt{3},
& \sqrt{3},
& -\sqrt{3},
& 0 \\ 
\sqrt{3},
& -\sqrt{3},
& -\sqrt{3},
& \sqrt{3},
& 0 \\ 
2,
& 2,
& 0,
& 0,
& -2 \\ 
\end{pmatrix}
\nonumber\\
&
\begin{tabular}{ |c||c|c|c|c|c|}
 \hline 
 & $\one$  & $e$  & $m$  & $m_1$  & $q$ \\ 
\hline 
 \hline 
$\one$  & $ \one$  & $ e$  & $ m$  & $ m_1$  & $ q$  \\ 
 \hline 
$e$  & $ e$  & $ \one$  & $ m_1$  & $ m$  & $ q$  \\ 
 \hline 
$m$  & $ m$  & $ m_1$  & $ \one \oplus q$  & $ e \oplus q$  & $ m \oplus m_1$  \\ 
 \hline 
$m_1$  & $ m_1$  & $ m$  & $ e \oplus q$  & $ \one \oplus q$  & $ m \oplus m_1$  \\ 
 \hline 
$q$  & $ q$  & $ q$  & $ m \oplus m_1$  & $ m \oplus m_1$  & $ \one \oplus e \oplus q$  \\ 
 \hline 
\end{tabular}
\end{align}
and
\begin{align}
&\ \ \ \ 
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$JK_4$ & $\one$ 
& $e$ 
& $m$ 
& $m_1$ 
& $q$ 
\\ 
\hline
$s$: & $0$
& $0$
& $\frac{1}{8}$
& $\frac{5}{8}$
& $\frac{2}{3}$
\\ 
\hline
$d$: & $1$
& $1$
& $\sqrt{3}$
& $\sqrt{3}$
& $2$
\\ 
\hline
\end{tabular}
\nonumber\\
S= & \begin{pmatrix}
1,
& 1,
& \sqrt{3},
& \sqrt{3},
& 2 \\ 
1,
& 1,
& -\sqrt{3},
& -\sqrt{3},
& 2 \\ 
\sqrt{3},
& -\sqrt{3},
& -\sqrt{3},
& \sqrt{3},
& 0 \\ 
\sqrt{3},
& -\sqrt{3},
& \sqrt{3},
& -\sqrt{3},
& 0 \\ 
2,
& 2,
& 0,
& 0,
& -2 \\ 
\end{pmatrix}
\nonumber\\
&
\begin{tabular}{ |c||c|c|c|c|c|}
 \hline 
 & $\one$  & $e$  & $m$  & $m_1$  & $q$ \\ 
\hline 
 \hline 
$\one$  & $ \one$  & $ e$  & $ m$  & $ m_1$  & $ q$  \\ 
 \hline 
$e$  & $ e$  & $ \one$  & $ m_1$  & $ m$  & $ q$  \\ 
 \hline 
$m$  & $ m$  & $ m_1$  & $ \one \oplus q$  & $ e \oplus q$  & $ m \oplus m_1$  \\ 
 \hline 
$m_1$  & $ m_1$  & $ m$  & $ e \oplus q$  & $ \one \oplus q$  & $ m \oplus m_1$  \\ 
 \hline 
$q$  & $ q$  & $ q$  & $ m \oplus m_1$  & $ m \oplus m_1$  & $ \one \oplus e \oplus q$  \\ 
 \hline 
\end{tabular}
\end{align}
From the fusion $e\otimes e = \one$, we see that $e$ carries a $\Z_2$ charge.
From the $S$-matrix, we see that $m$ (and $m_1$) carries the 
corresponding $\Z_2$-flux.


The  $SU(2)_4\times \overline{SU(2)}_4$ SymTO and $\cD(S^{\,}_{3})$ SymTO can
have a gapped domain wall between them, which describes the breaking of the
$\Z_2^{\two \leftrightarrow r}$ self-dual symmetry and reduce the
$SU(2)_4\times \overline{SU(2)}_4$ SymTO and $\cD(S^{\,}_{3})$ SymTO.  The
domain wall is caused by the condensation of $e \bar e$ in $SU(2)_4\times
\overline{SU(2)}_4$ SymTO (and no  condensation in the $\cD(S^{\,}_{3})$
SymTO).  More precisely, the  domain wall is described by the following
condensible algebra:
\begin{align}
\cA &=  
(\one,\one,\one)
\oplus (e,\bar e,\one)
\oplus (\one,\bar e,\one')
\oplus (e,\one,\one')
\oplus (q,\bar q,\two)
\oplus (q,\bar q,r)
\oplus (\one,\bar q,r_1)
\oplus (e,\bar q,r_1)
\nonumber\\ &\ \ \ \
\oplus (q,\one,r_2)
\oplus (q,\bar e,r_2)
\oplus (m,\bar m,s)
\oplus (m_1,\bar m_1,s)
\oplus (m,\bar m_1,s_1)
\oplus (m_1,\bar m,s_1)
\end{align}

The term  $(\one,\bar e,\one')$ in $\cA$ means that the anyon $\one'$ in
$\cD(S^{\,}_{3})$ SymTO and the anyon $\one\otimes \bar e=\bar e$ in
$SU(2)_4\times \overline{SU(2)}_4$ SymTO can condense in the domain wall.  In
other words, after going through the domain wall, the $\bar e$-anyon  in
$SU(2)_4\times \overline{SU(2)}_4$ SymTO turns into the $\one'$-anyon in
$\cD(S^{\,}_{3})$ SymTO.  Similarly, the term  $(e,\one,\one')$ in $\cA$ means
that,  after going through the domain wall, the $e$-anyon  in $SU(2)_4\times
\overline{SU(2)}_4$ SymTO turns into the $\one'$-anyon in $\cD(S^{\,}_{3})$
SymTO.  Thus the $e$-anyon and  the $\bar e$-anyon  in $SU(2)_4\times
\overline{SU(2)}_4$ SymTO carries the $\Z_2$-charge of the $S_3=\Z_3\rtimes
\Z_2$ symmetry.  The corresponding $\Z_2$-flux is carries by $m\bar m$-anyon in
$SU(2)_4\times \overline{SU(2)}_4$ SymTO, which has a $\pi$-mutual statistics
with both $e$-anyon and  $\bar e$-anyon.  This is also consistent with the term
$(m,\bar m,s) $ in $\cA$, which implies that after going through the domain
wall, the $m\bar m$-anyon  in $SU(2)_4\times \overline{SU(2)}_4$ SymTO turns
into the $s$-anyon (the $\Z_2$-flux) in $\cD(S^{\,}_{3})$ SymTO.  Thus, the
string operator that creates a pair of  $m\bar m$-anyons generates the $\Z_2$
(of $S_3$) transformation.

The Abelian anyon $e\bar e$ in $SU(2)_4\times \overline{SU(2)}_4$ SymTO does
not carries the $\Z_2$ charge of the $S_3$.  But it carries the $\Z_2^{\two
\leftrightarrow r}$ charge of the self-dual symmetry.  This is consistent with
the fact that the condensation $\cA= \one\oplus e\bar e$ reduces the
$SU(2)_4\times \overline{SU(2)}_4$ SymTO to $\cD(S^{\,}_{3})$
SymTO:\cite{CW220506244,CJW221214432,BBS231217322}
\begin{align}
 (SU(2)_4\times \overline{SU(2)}_4)_{/\one\oplus e\bar e}=
\cD(S^{\,}_{3}).
\end{align}
To summarize, the
anyons in $SU(2)_4\times \overline{SU(2)}_4$ and $\cD(S^{\,}_{3})$
SymTOs have the following relation
\begin{align}
\label{SymTOSymTO}
 e\bar e \to \one,\ \ \
 e \to \one',\ \ \
 \bar e \to \one',\ \ \
 m\bar m \to s,\ \ \
 q\bar q \to \two,\ \ \
 q\bar q \to r,\ \ \
 q \to r_1,\ \ \
 \bar q \to r_2 .
\end{align}


Since $e\bar e$ has $\pi$-mutual statistics with $m$ and $\bar m$ in
$SU(2)_4\times \overline{SU(2)}_4$ SymTO, thus $m$ and $\bar m$ are $\Z_2^{\two
\leftrightarrow r}$-flux for the self-dual symmetry.  In other words, the
string operator that creates a pair of  $m$-anyons generates the self-dual
transformation.  Similarly, the string operator that creates a pair of  $\bar
m$-anyons also generates the self-dual transformation.  However, the two
transformations differ by a $\Z_2$ transformation.  Because $m$'s quantum
dimension is $\sqrt 3$, the transformation generated by the string operator of
$m$ is an intrinsic non-invertible symmetry.

\begin{figure}[t!]
	\centering
	\includegraphics[height=1.0in]{FIGURES/QFTS3}
\ \ \ \ \
	\includegraphics[height=1.0in]{FIGURES/QFTRepS3}
	\caption{Isomorphic holographic discomposition
$(\eps, \t \cR)$
introduced in Ref. \cite{KZ150201690,KZ200308898,KZ200514178} 
exposes the symmetry and the SymTO of the model. 
See also Ref. \cite{ABS211202092,FT220907471}.
(Left) The $\cA_{S_3}$-condensation induced
topological boundary and the bulk $SU(2)_4\times \overline{SU(2)}_4$  SymTO
give rise to $S_3$-symmetry plus the self-dual symmetry.
(Right) The $\cA_{\cRep(S_3)}$-condensation induced
topological boundary and the bulk $SU(2)_4\times \overline{SU(2)}_4$  SymTO
give rise to $\cRep(S_3)$-symmetry plus the self-dual symmetry.
		}
	\label{fig:QFTS3}
\end{figure}


The $SU(2)_4\times \overline{SU(2)}_4$ SymTO has two
Lagrangian condensible algebras:
\begin{align}
\label{LcAlg}
\cA_{\cRep(S^{\,}_{3})} &=  (\one,\one)
\oplus (e,\bar e)
\oplus (m,\bar m)
\oplus (m_1,\bar m_1)
\oplus (q,\bar q)
\nonumber\\
\cA_{S_3} &=  (\one,\one)
\oplus (\one,\bar e)
\oplus (e,\one)
\oplus (e,\bar e)
\oplus 2(q,\bar q).
\end{align}
Thus, there are only two symmetries that give rise to the $SU(2)_4\times
\overline{SU(2)}_4$ SymTO.  Using \eqref{SymTOSymTO}, we see that the
$\cA_{S_3}$-condensation corresponds to the condensation of $S_3$-charges
$\one'$ and $\two$, as well as the condensation of $\Z_2^{\two \leftrightarrow
r}$-charge of the self-dual symmetry.  This leads us to conjecture that
$\cA_{S_3}$ gives rise to the $S_3$-symmetry plus the self-dual symmetry, {\it
i.e.} the symmetry of the self-dual $S_3$ symmetric model studied in Section
\ref{sec:S3model} (see Fig. \ref{fig:QFTS3}(left)).

Similarly, $\cA_{\cRep(S_3)}$-condensation corresponds to the condensation of
$S_3$-flux $s$ and $r$, as well as the condensation of $\Z_2^{\two
\leftrightarrow r}$-charge of the self-dual symmetry.  This leads us to
conjecture that $\cA_{\cRep(S_3)}$ gives rise to the $\cRep(S_3)$-symmetry plus
the self-dual symmetry, {\it i.e.} the symmetry of the self-dual $\cRep(S_3)$
symmetric model studied in Section \ref{sec:RepS3model} (see Fig. \ref{fig:QFTS3}(right)).

Using the Symmetry-Topological-Order correspodnece, we can classify the gapped
phases of the self-dual $S_3$ symmetric model, which is modeled by Fig.
\ref{fig:QFTS3}(left) with $\t\cR$ boundary given by the
$\cA_{S_3}$-condensation.  The gapped phases of the self-dual $S_3$ symmetric
model is given by gapped boundary $QFT_\text{ano}$, which is induced by
Lagrangian condensible algebras in \eqref{LcAlg}.  So the self-dual $S_3$
symmetric model has only two gapped phases.  If the  boundary $QFT_\text{ano}$
is induced by $\cA_{\cRep(S_3)}$-condensation, then the ground state degeneracy
is given by the inner product of the
two Lagrangian condensible algebras that induce the $\t \cR$ and
$QFT_\text{ano}$ boundaries:
\begin{align}
 GSD = (\cA_{S_3},\cA_{\cRep(S_3)}) = 4.
\end{align}
Here the  inner product $ (\cA_{S_3},\cA_{\cRep(S_3)})$ is defined by viewing
condensible algebra as integral vector whose components are the integral
coefficients in front of anyons in the expension of $\cA$.  This gapped phase
is a degeneracy of the $\Z_2$-state (with GSD = 3) and the $S_3$-state (with
GSD = 1) of the $S_3$ symmetric model.
The second gapped phase of the self-dual $S_3$ symmetric model is given by
$QFT_\text{ano}$ boundary induced  by $\cA_{S_3}$-condensation.
The ground state degeneracy
is given by 
\begin{align}
 GSD = (\cA_{S_3},\cA_{S_3}) = 8.
\end{align}
The second gapped phase is a degeneracy of the $\Z_3$-state (with GSD = 2) and
the $\Z_1$-state (with GSD = 6) of the $S_3$ symmetric model.
We see that the self-dual $S_3$ symmetric model does not have any gapped phase
with non-degenerate ground state.  Thus the combined $S_3$ and self-dual
symmetries is an anomalous symmetry.

Similarly, the self-dual $\cRep(S_3)$ symmetric model is given by Fig.
\ref{fig:QFTS3}(right), with $\t\cR$ boundary given by the
$\cA_{\cRep(S_3)}$-condensation. 
The  self-dual $\cRep(S_3)$ symmetric model also has only two gapped
phases, with ground state degeneracy:
\begin{align}
 GSD = (\cA_{S_3},\cA_{\cRep(S_3)}) = 4,\ \ \ \ \
 GSD = (\cA_{\cRep(S_3)},\cA_{\cRep(S_3)}) = 5.
\end{align}
Again, the self-dual $\cRep(S_3)$ symmetric model does not have any gapped
phase with non-degenerate ground state.  Thus the combined $\cRep(S_3)$ and
self-dual symmetries is an anomalous symmetry.






for the phase
diagram of $S^{\,}_{3}$ symmetric theories. In particular, any phase transition
between an $S^{\,}_{3}$-ferromagnet phase and an
$S^{\,}_{3}$-broken-down-to-$\Z^{\,}_3$ phase must be enriched by a
self-duality symmetry associated by this anyon permutation. A similar
self-duality symmetry enriches any phase transition between an $S^{\,}_{3}$
paramagnet phase and an $S^{\,}_{3}$-broken-down-to-$\Z^{\,}_2$ phase. In this
work, we discuss this duality in concrete terms for both $S^{\,}_{3}$ and
$\cRep(S^{\,}_{3})$ symmetries as realized in lattice models. We find that this
duality can be understood as gauging the $\Z^{\,}_3$ normal subgroup of
$S^{\,}_{3}$ in the $S^{\,}_{3}$-symmetric lattice model, while it corresponds
to gauging by the $\one \oplus \bm{2} $ algebra object in the
$\cRep(S^{\,}_{3})$-symmetric lattice model.

\AC{To add discussion of enlarged SymTO on the duality-symmetric lines.}


==> SECTIONS/introduction240516.tex <==
\section{Introduction}
\label{sec:intro}

In quantum many-body physics, global internal symmetries are conventionally
represented by unitary (or anti-unitary) operators that act non-trivially on
all degrees of freedom, everywhere in space.  The elementary charged objects
under such symmetries are local operators with support over a finite region of
space.  

This conventional picture of symmetries was recently generalized in several
directions. For example, the symmetry transformations were generalized to act on
lower dimensional subspaces \cite{NOc0605316,NOc0702377} with the elementary charged
objects being higher dimensional~\cite{GKW14125148,KT170108264}.  In the language
of field theory, a $p$-form symmetry is generated by $(d-p)$-dimensional, \ie
co-dimension $p$, topological defects that can be inserted into the partition
functions of theories defined on $(d+1)$ spacetime dimensions. The
corresponding charges then live in a $(p+1)$-dimensional worldsheet in
spacetime. The conventional global internal symmetries correspond to the case
of $p=0$. The mathematical structure that captures a collection of several
higher-form symmetries of different order is that of a \emph{higher-group}: a
$p$-group involves $0$-form through $(p-1)$-form symmetries.  Higher-form
symmetries can be treated within Hamiltonian formalism as well, by choosing a
time slice together with a corresponding Hilbert space.  Then higher-form
symmetry operators acting on this Hilbert space are defined by restricting to
the topological defects that are supported only on the time slice.
% { \blue See Refs.\ \blue cite here that study the realizations of higher-form
% symmetries.} 
Although typical lattice models for condensed matter systems do not have
higher-group symmetries, they can appear as emergent
symmetries \cite{W181202517} or even \emph{exact emergent} symmetries 
at low energies \cite{PW230105261,PW231008554}.


In many ways, higher-form symmetries behave just like ordinary symmetries: they
can be spontaneously broken leading to degenerate ground states or Goldstone
bosons \cite{NOc0702377,L180207747}, depending on whether the symmetry is
discrete or continuous; they can have 't Hooft anomalies themselves, or have
mixed 't Hooft anomalies with crystalline symmetries leading to
Lieb-Schultz-Mattis (LSM)-type theorems \cite{KSR180505367}; they can lead to
new symmetry protected topological (SPT) phases \cite{KT13094721,Y150803468}.
A generic way to construct models with higher-form symmetries in (2+1) dimensions and higher, is via
gauging (some subgroup of) an ordinary symmetry
\cite{JW191213492,MAT230701266}.

A further generalization of symmetries comes 
from considering operators that commute with the Hamiltonian 
but are not invertible, and hence have non-trivial kernels.
These are the so-called non-invertible symmetries~\cite{TW191202817}.
The composition law, or fusion rule, of these symmetry operators does not satisfy a group-like multiplication rule. 
Instead, given two non-invertible symmetry
operators, their fusion results in a sum of 
symmetry operators which may be invertible or non-invertible.
When the symmetries of the system form a finite collection,
the structure that unifies invertible and non-invertible
0-form and higher-form symmetries is that of a fusion higher category $\mathcal{C}$~\cite{KZ200514178,FMT220907471}. 
In $(d+1)$ spacetime dimensions, $\cC$ is a fusion $d$-category.
In this work, we will focus on $(1+1)$ dimensions
so that the symmetry structure is described by ordinary fusion categories, 
instead of fusion higher categories.
In this case, symmetry operators in a fusion category $\mathcal{C}$ 
are labeled by the simple objects $\mathsf{a}$ of $\mathcal{C}$.
The fusion of two symmetry operators $\widehat{W}^{\,}_{\mathsf{a}}$ and 
$\widehat{W}^{\,}_{\mathsf{b}}$, labeled by objects $\mathsf{a}$ and 
$\mathsf{b}$ delivers the sum
\begin{align}
\widehat{W}^{\,}_{\mathsf{a}}\,
\widehat{W}^{\,}_{\mathsf{b}}
=
\sum_{\alpha}
\mathrm{N}^{\mathsf{c}}_{\mathsf{a}\,\mathsf{b}}\,
\widehat{W}^{\,}_{\mathsf{c}},
\end{align}
where integers $\mathrm{N}^{\mathsf{c}}_{\mathsf{a}\,\mathsf{b}}$ 
are the \emph{fusion coefficients}.

Non-invertible symmetries were explored in the realm of quantum field theory
(QFT) in the form of topological defect lines of $(1+1)d$ rational conformal
field theories
(RCFT)~\cite{V8860,MS8977,FFIS0404051,FSh0607247,FGRS07053129,FS09095013}.
More recently, such topological defect lines have been established as
non-invertible symmetries within the framework of generalized
symmetries~\cite{BT170402330,T171209542,TW191202817}. 
% In Ref.
% \cite{KZ200308898,KZ200514178}, a general classifying theory of anomaly-free
% non-invertible symmetries (referred to as algebraic higher symmetries) in $d$-dimensional space was given in terms of
% local fusion $d$-category, which describe the fusion and braiding of the
% symmetry charges, that can be point-like, string-like, or higher-dimensional). 
% The
% generalized symmetries
% can also be described and classified by topological orders in one higher
% dimension (up to holo-equivalence)~\cite{KZ200308898,KZ200514178,FT220907471}.
They have found applications in various QFT contexts~\cite{KS200807567,CLS220505086,CO220506243}.  Realizations of
non-invertible symmetries and phases of matter with these symmetries in lattice
models are far less understood.  On the one hand, the long-distance and
low-energy limit -- usually referred to as the infrared (IR) limit -- of many
body quantum systems  often have an effective QFT description. Since by now we
know many examples of QFTs that possess non-invertible symmetries, one expects
that there is a natural place for such symmetries in many body physics, \eg in
labeling the symmetry structure of the zero temperature phases of many-body
quantum systems. On the other hand, na\"ive lattice regularization of QFTs may
break emergent symmetries of the continuum theory (see, \eg \Rf{GLS210301257}).
In that spirit, it is desirable to construct lattice models that respect
generalized symmetries, putting them on the same footing as ordinary
symmetries. To be precise, by ``lattice model'' we mean local Hamiltonians
acting on a Hilbert space that is a tensor product of finite-dimensional local
Hilbert spaces -- we will refer to such lattice models, somewhat glibly, as
``spin chains".  We will require that the lattice Hamiltonians we construct
possess certain non-invertible symmetries, \ie they commute with such
non-invertible symmetry operators. 

One strategy to obtain non-invertible symmetries is to
start from a model with ordinary (finite) non-Abelian $G$ symmetry and
gauge it.  In the resulting gauge theory, in $d+1$ spacetime dimensions, the Wilson
loops obey the fusion rules dictated by the representations of $G$ and form a
fusion (higher) category $d$-$\cRep(G)$, which is not group-like whenever $G$ is
non-Abelian.  This strategy was used to construct various lattice models with
non-invertible symmetries~\cite{JW191213492,DT180210104,LV211209091}.  
Another class of examples can be obtained through the so-called half-gauging
scheme. Namely, if gauging an invertible symmetry of a theory $\cT$ produce an
isomorphic dual symmetry, a defect constructed by gauging this symmetry 
on one half of spacetime, the interface can be thought of 
as a non-invertible self-duality defect~\cite{KOZ211101141,CCS211101139,CCS220409025}.
Bootstrapping off of this, it is also possible to construct new duality
by half-gauging non-invertible symmetries~\cite{DLW231117044,CLS231019867}.
On a related note, statistical mechanical models with general fusion 
category symmetries were proposed and studied in 
\Rfs{AFM200808598,AMF160107185}.
Recently, non-invertible self-duality symmetries in lattice models have also 
been obtained by gauging internal symmetries that
participate in a mixed anomaly with translation symmetry such as in the case of
Lieb-Schultz-Mattis (LSM) anomalies~\cite{SS230702534,S230805151,SSS240112281}. 
It was also shown that non-invertible symmetries appear generically as emergent symmetries 
in ordered phases associated with SSB of ordinary symmetries~\cite{P230805730}.

A different perspective on finite generalized symmetries was proposed 
in~\Rfs{JW190513279,JW191213492}; the authors argued that such 
symmetries can be viewed as special kinds of non-invertible gravitational
anomalies. In other words, symmetry data can be stored in a non-invertible
field theory in one higher dimension such that the physical theory with
generalized symmetries is realized as a boundary theory of the former.
% It is well-known that gravitational anomalies are invariant under 
% renormalization group flow, and hence can constrain low-energy dynamics,
% in much the same way that symmetries do.
This leads to a holographic theory of generalized symmetries in terms of 
topological orders in one higher
dimension~\cite{KZ150201690,KZ200308898,KZ200514178,ABS211202092,FT220907471}.
This idea goes by various names: symmetry-topological-order (SymTO)
correspondence~\cite{KZ150201690,KZ200308898,KZ200514178},\footnote{SymTO was referred to as
``categorical symmetry'' in some early
papers~\cite{JW191213492,KZ200308898,KZ200514178}. 
In present literature,
categorical symmetry is used to refer to non-invertible symmetry (referred to as algebraic higher symmetry in \Rf{KZ200514178}).  See
\app{app:SymTO} for a brief review of SymTO.}
symmetry-topological-field-theory (SymTFT)~\cite{ABS211202092},
topological symmetry \cite{FT220907471}, or
topological holography~\cite{MMT220710712,HC231016878,WYP240419004}. 


Generalized symmetries can also be viewed from the perspective of the
algebra of a subset of all local operators. Given a set of symmetry 
transformations, the subset of local operators invariant under these 
transformations forms the algebra of local symmetric operators (also 
called a bond algebra~\cite{CON09070733,CON11032776}). 
One can turn this idea on its head and consider subsets of local operators 
as (indirectly) defining a generalized symmetry, provided the subset forms 
an algebra. \Rf{CW220303596} took this point view and showed that
isomorphic algebras of local symmetric operators correspond one-to-one to
topological orders in one higher dimension, by considering simple examples.
The commutant algebra of the subset of local operators contains operators
that implement (generalized) symmetry transformations~\cite{MM210810324,MM220903370}.  
The structure of commutant algebras is rich enough to include the
above-mentioned non-invertible symmetries.
Notably, this structure is less rigid than that of fusion
(higher) categories since the fusion coefficients need not be non-negative
integers. Making contact between the commutant algebraic approach and
the topological defect approach of generalized symmetries is an 
interesting open question.

There has been an exciting flurry of recent work
\cite{KZ200308898,KZ200514178,I211012882,LV211209091,LDV221103777,DT230101259,BBS231003784,FTA231209272,SSS240112281}
exploring gapped phases of systems with fusion category symmetries.
A generalized Landau paradigm \cite{CW220506244,CJW221214432,BBS231217322},
classifying both gapped and gapless phases in systems with general fusion
category symmetries in 1+1D has been formulated based condensable algebra in
the topological order in one higher dimension.  These results were obtained
within the frameworks of SymTO~\cite{CW220506244,CJW221214432}, SymTFT~\cite{ABS211202092}, and topological
symmetry~\cite{FT220907471}.

In this paper, we contribute to this rapidly developing literature by exploring the possible phases, gapped or gapless, and continuous phase transitions realized in \emph{spin chains} with non-invertible symmetries. In particular, we study the example of the smallest anomaly-free symmetry category: $\cRep(S_3)$. Building up to that,
in Sec.\ \ref{sec:S3model} we introduce 
a spin chain with $S^{\,}_{3}$ symmetry constructed out of qubit and qutrit degrees of freedom. 
% Since this symmetry is anomalous, the system is required to be symmetric gapless or gapped with degenerate ground states owing to spontaneous breaking of the symmetry. We identify multiple gapless states in the KW-symmetric manifold in the parameter space of our Hamiltonian. 
In Sec.\ \ref{sec:RepS3model}, we show how gauging either the entire $S^{\,}_{3}$ symmetry or its non-normal
$\mathbb{Z}^{\,}_{2}$ subgroup delivers a spin chain with $\cRep(S^{\,}_{3})$ symmetry.
By studying appropriate limits, we identify fixed-point ground states corresponding to the four distinct $\cRep(S^{\,}_{3})$ spontaneous symmetry breaking (SSB) patterns.
We explore the phase diagrams of both spin chains using tensor network algorithms to verify the analytical predictions.
Section \ref{sec:symTO} is a synthesis
of the salient aspects of our results from the point of view of the SymTO framework.  
In section \ref{sec:disc} we discuss connections of our results with more abstract approaches, propose order 
parameters that detect SSB patterns in our models,
and comment on an incommensurate gapless phase that our numerical calculations reveal.
We close with some comments on directions for future exploration in Section~\ref{sec:conclusion}.

{\blue ************** The alternative introduction *****************}



\subsection*{Relation to prior literature}

\subsection*{Summary of the main results}

\begin{enumerate}[(i)]
\item 
We show, through a microscopic calculation, that our spin chain \eqref{eq:def Ham gen S3} with 
$S^{\,}_3$ symmetry is dual to the $\cRep(S^{\,}_{3})$-symmetric spin chain \eqref{eq:def Ham gen RepS3}  
by gauging a 
$\Z^{\,}_{2}$ subgroup of $S^{\,}_{3}$.
As a consequence, phase diagrams of these spin chains can be mapped to each other in a one-to-one manner.
% Therefore, their respective phase diagrams have the same shape in that the gapped and gapless 
% phases can be matched, even though ground state degeneracies and spontaneous symmetry breaking (SSB)
% patterns do not.

\item 
We find gapped phases realizing all four SSB patterns of both
$S^{\,}_{3}$ and $\cRep(S^{\,}_{3})$ symmetries which correspond to the four inequivalent
module categories over the corresponding fusion categories~\cite{TW191202817}.
We define order and disorder operators whose non-vanishing expectation values 
can be used to distinguish different SSB patterns. 
For the non-invertible $\cRep(S^{\,}_{3})$ symmetry, the SSB is detected 
by string order parameters as opposed to the invertible $S^{\,}_{3}$ symmetry.

\item 
We show that for special subspaces in the parameter space, our spin chains 
are both invariant under an exact (intrinsic) non-invertible 
self-duality symmetry~\cite{KOZ220911062,KZZ220501104}. 
We provide the lattice operators that implement the respective 
self-duality symmetry in the form of a sequential circuit.\footnote{Notably, 
\Rf{CDZ230701267} considered this class of sequential circuits as maps between
distinct gapped phases.}
In particular, for the
$\cRep(S^{\,}_{3})$-symmetric model \eqref{eq:def Ham gen RepS3},
this circuit implements a self-duality symmetry associated with gauging $\cRep(S^{\,}_{3})$
by the algebra object $\one\oplus\two$.


\item 
For both spin chains, the four gapped phases meet at a multi-critical
point that is symmetric under the respective non-invertible self-duality 
symmetry. For each multi-critical point, we identify three relevant perturbations,
two of which break the non-invertible self-duality symmetry explicitly. 
In particular, for the $S^{\,}_3$ spin chain, one of these relevant perturbations 
allows the realization of a (Landau-forbidden) direct continuous transition 
between SSB phases preserving $\Z^{\,}_3$ and $\Z^{\,}_2$ subgroups.

\item 
We find an extended gapless region in the 
parameter space which is consistent with an incommensurate gapless phase. 
% This 
% phase has low-energy excitations carrying incommensurate quasi-momenta. 
To better understand
this gapless phase, we draw an analogy with an exactly solvable spin-1/2 chain with 
exact $\Z^{\,}_{2}$ KW self-duality symmetry. This spin chain, also supports a 
gapless incommensurate phase with central charge $c=1$ 
and an anomalous chiral $\mathrm{U}(1)$ symmetry\footnote{In the low-energy CFT description, only the left-movers 
carry the $\mathrm{U}(1)$ charge while the right-movers are described by two branches of Majorana fermion
fields with different velocities.} that emanates~\cite{CS221112543} from
lattice translation symmetry.\footnote{
Along the self-dual line, the Majorana representation of translation symmetry carries an
LSM anomaly since there are odd number of Majorana degrees of freedom per unit cell,
see Refs.\ \cite{HHG160408591,ATM210208389,SS230702534}.
}
This gapless phase is separated from the neighboring gapped phases by critical
lines with dynamical critical exponent $z>1$. 
We provide arguments on why this feature may be valid for incommensurate phases more generally.
% An incommensurate phase contains $U(1)$ current and has a central charge $(c,\bar c) \geq (1,1)$.
% The continuous transition between
% incommensurate phase and gapped commensurate phase is described by a critical
% point with dynamical critical exponent $z>1$.
We also discover a new type of continuous  transition in the incommensurate phase.
The new continuous transition has the same number of gapless modes at and away from the transition point.\footnote{The number of gapless mode can be measured experimentally, via the the thermal conductance of short clean sample.}
In our example, there is only one $U(1)$ current $J_L$ for left-movers at the transition point, while there are two $U(1)$ currents $J_L,J_R$ for for both left- and right-movers away from the transition point.

\item 
We identify the SymTO of our self-dual $S^{\,}_3$ and $\cRep(S^{\,}_3)$-symmetric spin chains to be the
2+1D $\mathrm{JK}^{\,}_{4}\boxtimes \overline{\mathrm{JK}^{\,}}_4$ topological order. 
We also obtain possible phases and phase transitions of the self-dual spin chains from the allowed boundary conditions of the SymTO. In particular, we show that
the self-dual spin chains do not allow gapped non-degenerate ground states, consistent with the fact that the non-invertible self-duality  symmetries are anomalous.

\end{enumerate}


\textbf{Note added:} While this manuscript was being completed, 
we became aware of potentially overlapping work in Refs.\ \cite{BBST1,BBST2}; 
we thank the authors for coordinating their arXiv submission with us.

